Visual Foresight Trees for Object Retrieval from Clutter with Nonprehensile Rearrangement

This paper considers the problem of retrieving an object from many tightly packed objects using a combination of robotic pushing and grasping actions. Object retrieval in dense clutter is an important skill for robots to operate in households and everyday environments effectively. The proposed solution, Visual Foresight Trees (VFT), intelligently rearranges the clutter surrounding a target object so that it can be grasped easily. Rearrangement with nested nonprehensile actions is challenging as it requires predicting complex object interactions in a combinatorially large configuration space of multiple objects. We first show that a deep neural network can be trained to accurately predict the poses of the packed objects when the robot pushes one of them. The predictive network provides visual foresight and is used in a tree search as a state transition function in the space of scene images. The tree search returns a sequence of consecutive push actions yielding the best arrangement of the clutter for grasping the target object. Experiments in simulation and using a real robot and objects show that the proposed approach outperforms model-free techniques as well as model-based myopic methods both in terms of success rates and the number of executed actions, on several challenging tasks. A video introducing VFT, with robot experiments, is accessible at https://youtu.be/7cL-hmgvyec. The full source code is available at https://github.com/arc-l/vft.

==> texs/01-intro.tex <==

AAAAAAA.

\begin{figure}[ht!]
    \centering
    \subfloat[]{
        \includegraphics[width = \linewidth]{example-image-a}\label{fig:intro-setup}
    }
    
    \subfloat[]{
        \includegraphics[width = \linewidth]{figures/system-high-level.pdf}\label{fig:intro-system}
    }
    \caption{\label{fig:intro}
        What?
    }
\end{figure}

==> texs/05-methods.tex <==
In this section, we first illustrate the overall workflow of the system, which includes three main modules, which are the grasp network for grasping, Push prediction (DIPN) network for predicting the post scene after a push action, MCTS~\cite{mcts2012} that uses Grasp Network as the reward function of each state, also DIPN~\cite{huang2020dipn} as the transition function between parent node and the child node. With integrated pipeline, we are able to solve the problem efficiently.

\subsection{Grasp Network Adaption}
The Grasp Network we are using is from the previous work~\cite{huang2020dipn}, which is similar to the DQN for grasping as presented in~\cite{zeng2018learning}.
The Grasp Network takes the state observation $o$ as the input, and outputs a pixel wised grasp Q value $Q_g$. 
$Q_g$ is a one channel image with same size as the $o$, and the Q value in $Q_g$ represents the predicted reward if the robot grasps at the corresponding position.
The Q value is a single-step grasp reward, defined as 1 for a successful grasp and 0 otherwise. 
Since we are all care about the target object, the successful grasp is defined as that an object is grasped and the object is the target object.

The output $Q_g$ contains an assumption that is the orientation of the grasp is fixed, the left finger is on the left hand side of the pixel and right finger is on the right hand side as shown in Fig ?. 
To produce the orientation $\theta$ required for a grasp action, the state observation $o$ is rotated evenly distributed 16 times between 0 and 360 degrees, before passing to the Grasp Network.
As a result, we have 16 grasp pixel wised $G_{g_i}$ ($i$ is an integer from 1 to 16), we use $Q_{g_{A}}$ to denote all of them.
For grasping, the greedy strategy is applied here, a single pixel the $\max Q_{g_{A}}$ is chosen, the pixel position $(x_i, y_i)$ in the corresponding $G_{g_i}$ is recorded, and will be transformed back as $(x, y)$ based on the rotation angle $\theta$ applied to $o$. The $o$ contains a depth image, the depth value $z$ can be obtained according to $(x, y)$. That is a grasp action $a^(grasp) = (x, y, z \theta)$ is acquired.

The main difference compared to the previous work is the objective and the learning strategy. 
The objective in the previous work~\cite{zeng2018learning, huang2020dipn} are grasping all the objects, which is not the case in this paper, we only grasp the target object. Only given rewards to the target object would be a straight forward adaption as implemented in~\cite{xu2021efficient}. Nevertheless, for faster training, and high accuracy, xu2021efficient

\subsection{Push Prediction (DIPN)}
\subsection{Monte Carlo Tree Search Implementation}

